Probing the anomalous tqgamma couplings in photon-proton collisions

The top quark flavor changing neutral current processes are extremely suppressed within the Standard Model. Nevertheless, they could be enhanced in a new physics model beyond the Standard Model. Investigating the top quark's flavor changing neutral current interactions at colliders would be an important test in terms of new physics. In this work, we examine the potentials of the processes ${e^{-}} {p} {\rightarrow} {e^{-}} {\gamma}^{*} {p} {\rightarrow} {e^{-}} W^{+} b {\gamma}^{*}{\rightarrow} {e^{-}} {j} {\bar{j}} b {\gamma}^{*} $ and ${e^{-}} {p} {\rightarrow} {e^{-}} {\gamma}^{*} {p} {\rightarrow} {e^{-}} W^{+} b {\gamma}^{*}{\rightarrow} {e^{-}} \textit{l} {\nu}_\textit{l} b {\gamma}^{*} $ at the FCC-eh with $\sqrt{s} = 7.08 $ and $ 10.0 TeV $ to study anomalous $tq\gamma$ couplings via effective Lagrangians. We obtain $95{\%}$ confidence level sensitivities on the anomalous coupling parameters at the three FCC-eh energies and various integrated luminosities. We find that our limits are at least two orders of magnitude better than the current LHC experimental results.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.

\end{thebibliography}


